PIONEER: Studies of Rare Pion Decays

A next-generation rare pion decay experiment, PIONEER, is strongly motivated by several inconsistencies between Standard Model (SM) predictions and data pointing towards the potential violation of lepton flavor universality. It will probe non-SM explanations of these anomalies through sensitivity to quantum effects of new particles even if their masses are at very high scales. Measurement of the charged-pion branching ratio to electrons vs. muons $R_{e/\mu}$ is extremely sensitive to new physics effects. At present, the SM prediction for $R_{e/\mu}$ is known to 1 part in $10^4$, which is 15 times more precise than the current experimental result. An experiment reaching the theoretical accuracy will test lepton flavor universality at an unprecedented level, probing mass scales up to the PeV range. Measurement of pion beta decay, $\pi^+\to \pi^0 e^+ \nu (\gamma)$, with 3 to 10-fold improvement in sensitivity, will determine $V_{ud}$ in a theoretically pristine manner and test CKM unitarity, which is very important in light of the recently emerged tensions. In addition, various exotic rare decays involving sterile neutrinos and axions will be searched for with unprecedented sensitivity. The experiment design benefits from experience with the recent PIENU and PEN experiments at TRIUMF and the Paul Scherrer Institut (PSI). Excellent energy and time resolutions, greatly increased calorimeter depth, high-speed detector and electronics response, large solid angle coverage, and complete event reconstruction are all critical aspects of the approach. The PIONEER experiment design includes a 3$\pi$ sr 25 radiation length calorimeter, a segmented low gain avalanche detector stopping target, a positron tracker, and other detectors. Using intense pion beams, and state-of-the-art instrumentation and computational resources, the experiments can be performed at the PSI ring cyclotron.

==> Appendices/Authors.tex <==

{\bf PIONEER Collaboration}


\author[23]{W. Altmannshofer}
\author[12]{H. Binney}
\author[28]{E. Blucher}
\author[2,3]{D. Bryman}
\author[6] {L. Caminada}
\author[6] {S. Corrodi}
\author[4]{S. Chen}
\author[5]{V. Cirigliano}
%\author[6,7,8]{A. Crivellin}
\author[9]{ S. Cuen-Rochin}
\author[10]{A. Czarnecki}
\author[19] {A. DiCanto}
\author[11]{L. Doria}
\author[29] {A. Fienbert}
\author[24] {A. Gaponenko}
\author[12]{A. Garcia}
\author[13]{L. Gibbons}
\author[14]{C. Glaser}
\author[11]{M. Gorchtein}
\author[15]{T. Gorringe}
\author[23]{S. Gori}
\author[23]{A. Grillo}
\author[12]{D. Hertzog}
\author[12]{ Z. Hodge}
\author[16]{ M. Hoferichter}
\author[18]{S.  Ito}
\author[17]{T. Iwamoto}
\author[19] {D. Jaffe}
\author[12]{ P. Kammel}
\author[12]{J. Kaspar }
\author[19] {S. Kettel}
\author[24] {B. Kiburg}
\author[6] {A. Knecht}
\author[26]{T. Koffas} 
\author[13]{ K. Labe}
\author[12]{J. LaBounty}
\author[6] {U. Langenegger}
\author[3]{ C. Malbrunot}
\author[19]{ W. Marciano}
\author[23] {S. M. Mazza}
\author[20]{ S. Mihara}
\author[3]{ R. Mischke}
\author[17]{T. Mori}
\author[19] {J. Mott}
\author[12] {E. Muldoon}
\author[3]{T. Numao }
\author[17]{ W. Ootani}
\author[1]{ C. Ortega Hernandez}
\author[3] {K. Pachel}
\author[14]{ D. Po\v{c}ani\'c}
\author[24]{C. Polly}
%\author[3] {F. Retiere}
\author[11] {D. Ries}
\author[12] {R. Roehnelt}
\author[21]{ D. Salvat}
\author[23] { B. Schumm}
\author[6] {P. Schwendimann}
\author[23] { A. Seiden}
\author[25] {A. Soter}
%\author[3] { A. Sher}
\author[27] {R. Shrock}
\author[22]{T. Sullivan}
\author[12] {D. Sweigart}
\author[19] {V. Tischenko}
\author[19] { A. Tricoli}
\author[3]{B. Velghe}
\author[17] {T. Wataru}
\author[12] {C. Welch}
\author[3] {V. Wong}
\author[19] {E. Worcester}




\affiliation[1]{Universidad Nacional Autonoma de Mexico}
\affiliation[2]{University of British Columbia}
\affiliation[3]{TRIUMF}
\affiliation[4]{Tsinghua University}
\affiliation[5]{Los Alamos National Laboratory}
\affiliation[6]{Paul Scherrer Institute}
\affiliation[7]{University of Zurich}
\affiliation[8]{CERN}
\affiliation[9]{Universidad Autonoma de Sinaloa}
\affiliation[10]{University of Alberta}
\affiliation[11]{Johannes Gutenberg University of Mainz}
\affiliation[12]{University of Washington}
\affiliation[13]{Cornell University}
\affiliation[14]{University of Virginia}
\affiliation[15]{University of Kentucky}
\affiliation[16]{University of Bern}
\affiliation[17]{University of Tokyo}
\affiliation[18]{Okayama University}
\affiliation[19]{Brookhaven National Laboratory}
\affiliation[20]{KEK}
\affiliation[21]{Indiana University}
\affiliation[22]{University of Victoria}
\affiliation[23]{University of California Santa Cruz}
\affiliation[24]{Fermilab }
\affiliation[25]{ETH Zurich}
\affiliation[26]{Carleton University}
\affiliation[27]{Stoney Brook University}
\affiliation[28]{University of Chicago}
\affiliation[29]{Pennsylvania State University}


==> Appendices/inTargetDifSuppression.tex <==
\section{In-target Decay-in-flight $\pi \rightarrow \mu \nu$ Suppression with BDT}
\label{sec:DIFsuppression_BDT_appendix}

\begin{itemize}
    \item plots of input features (pienu vs DIF)
    \item BDT score distribution
    \item ROC curve
    \item suppression factor with the consideration of energy smearing
\end{itemize}

==> PioneerExperiment/BeamSim.tex <==
\subsection{Beamline Simulations}
	
\subsubsection{Beamline Simulations and Optimization}
The PSI High Intensity Proton Accelerator (HIPA) chain consists of a Cockcroft-Walton pre-accelerator, delivering 870 keV protons to a set of two isochronous cyclotrons which further accelerate to the maximum 590 MeV. 
In the Ring cyclotron, the protons are accelerated by four copper resonator cavities operated in continuous wave (CW) mode at a frequency of 50.6 MHz, giving the periodic 19.75~ns beam microstructure and their final energy of 590 MeV.
The $\pi$E5 channel is a high-intensity low-energy muon and pion beamline, with a maximum momentum of 120~MeV/c, that views the second graphite production target, Target~E, at 165$^{\circ}$ with respect to the proton beam axis.
The $\pi$E5 channel is used exclusively for particle physics experiments, and is currently home to the MEG~II and Mu3e experiments.
The channel length from Target~E to end of the QSB43 quadrupole magnet and the entrance to the experimental area is 13~m, giving approximately 7~m of free space between the concrete wall and current MEG~II infrastructure.
In this area the SEP41 E$\times$B Wien Filter for particle separation, QSK quadrupole triplet for focusing the beam on the ATAR, and the PIONEER installation could be placed.
\begin{figure}[h]
	\centering
	\includegraphics[width=1\linewidth]{Figures/G4BLSIM_PiE5_Labeled.png}
	\caption{The G4beamline model of the $\pi$E5 beamline including a stand-in calorimeter. Important elements along the beamline where rates are compared are labeled.}
	\label{fig:g4blsim_pie5_labeled}
\end{figure}

Simulations for both pion production at Target~E and transport of particles down the $\pi$E5 channel are performed using the G4Beamline toolkit~\cite{Roberts:2008zzc}.
A figure of the $\pi$E5 beamline from the G4Beamline simulation, beginning at Target E and ending at the PIONEER calorimeter, is shown in \cref{fig:g4blsim_pie5_labeled}.
The pion production simulation utilizes the parameterized cross section developed for the High Intensity Muon Beamline (HiMB) project.
The absolute rates determined from the simulation for particles near the production target are shown in \cref{fig:productionrates}.
\begin{figure}[h]
	\centering
	\includegraphics[width=1\linewidth]{Figures/TgEProdSim_HiMBHYBRID_10B-PoT_MomSpecFromTarget_SF100_positive.pdf}
	\caption{The rates of positive charged particles produced at Target E with longitudinal momentum in the direction of the $\pi$E5 channel. }
	\label{fig:productionrates}
\end{figure}

The G4Beamline simulation was originally tuned for 28~MeV/c muons and has been rescaled for the respective pion momenta.
Some tuning was performed for the last two dipoles and quadrupole triplets to optimize transmission through the SEP41 and on to the ATAR.
Rates for pions and muons reaching the entrance to experimental area for beamline central momenta ranging from 55~MeV/c to 75~MeV/c are shown in \cref{fig:piE5rates}.
The rates for those particles reaching the entrance to the experimental area (QSB43) and 4.8~m downstream at the entrance to the calorimeter volume (CALO Entrance) at the lower and upper end of the possible momentum ranges are listed in \cref{tbl:rates_55MeVc} and \cref{tbl:rates_75MeVc}.  

\begin{figure}[h]
	\centering
	\includegraphics[width=1\linewidth]{Figures/AtQSB43DSPiE5_Rates_PionsMuons.png}
	\caption{The rates for pions and muons at the entrance to the experimental area (QSB43).}
	\label{fig:piE5rates}
\end{figure}

	\begin{center}
	\begin{tabular}{p{4cm}||p{3cm}|p{3cm}|p{3cm}} 
		\multicolumn{4}{c}{Particle Rates ($\times 10^{8}$) in $\pi$E5 (p$_{\pi^{+}}$=55 MeV/c) at 2.2~mA I$_{p}$} \\
		\hline
		Beamline Position& $\pi^{+}$ & $\mu^{+}$ & $e^{+}$\\
		\hline
		QSB43 & 0.50 & 1.22 & x\\
		CALO Entrance & 0.09 & 0.59 & x\\
	\end{tabular}
	\label{tbl:rates_55MeVc}
\end{center}

\begin{center}
	\begin{tabular}{p{4cm}||p{3cm}|p{3cm}|p{3cm}} 
		\multicolumn{4}{c}{Particle Rates ($\times 10^{8}$) in $\pi$E5 (p$_{\pi^{+}}$=75 MeV/c) at 2.2~mA I$_{p}$} \\
		\hline
		Beamline Position& $\pi^{+}$ & $\mu^{+}$ & $e^{+}$\\
		\hline
		QSB43 & 4.66 & 2.68 & x\\
		CALO Entrance & 1.10 & 1.34 & x\\
	\end{tabular}
    \label{tbl:rates_75MeVc}
\end{center}

The pion rates calculated in simulation at the entrance to the calorimeter are approximately a factor two lower than the latest measurements at $\pi$E5, nevertheless they exceed the requirements of the experiment by two orders of magnitude.
This high rate would allow for losses in the SEP41 or upstream collimation, necessary for reducing background events in the ATAR and calorimeter.
Verification of these rates from measurements and comparison to simulation will be critical in determining achievable pion rates at the ATAR.
\subsection{Beamline Studies}
	
	{\it AS: editing offline}

==> Planning/Cost.tex <==






Table~\ref{cost} indicates the estimated costs of the PIONEER experiment assuming that the MEG 1000~l LXe supply (estimated value CHF 7.5M) will be used. 

\begin{table}[htbp]
    \centering
    \begin{tabular}{p{3in}r}
    \toprule
    PIONEEER Cost Estimate & M ChF \\
    \hline
    R\&D & 2.0 \\
    ATAR & 1.3 \\
    Trackers/Beam instr. & 0.5 \\
    Calorimeter & 20.3 \\
    Trigger/DAQ & 1.0 \\
    Other & 1.0 \\
    {\bf Total} & {\bf 26.1} \\

    \bottomrule
    \end{tabular}
\caption{ PIONEER preliminary cost estimate.}
\label{cost}
\end{table}

%\begin{figure}[htbp]

%\centering
%\includegraphics[scale=0.5]{Figures/CostEstimate.pdf}
%\caption{ PIONEER preliminary cost estimate.}
%\label{cost}
%\end{figure}

==> Planning/Timeline.tex <==
\label{sec:timeline_estimate}
We present an optimistic schedule  for \nexp\ for the next several  years under the assumptions that program approval stages and external funding decisions are positive and proceed expeditiously: 

\begin{itemize}%[leftmargin=*]
\item 2022:  Submit experimental proposal to PSI and make R\&D requests to funding agencies (US, Japan, Europe, Canada);  initiate first lab tests of prototype devices; perform simulations and further develop the experiment design; beam properties test at PSI.
\item 2023--24:  Beamline studies, detector prototype development and  test beam measurements; technical design report; funding decisions.
\item 2025--27: Full-scale production of detectors, electronics, DAQ sub-systems; short physics integration runs of available subsystems.
\item 2028:  \nexp\ engineering run and first physics production.
\item 2029: Full-scale  physics measurement program.
\end{itemize} 


==> Planning/alphCollaboration.tex <==
\author{W.~Altmannshofer}\affiliation {University of California Santa Cruz}
\author{H.~Binney}\affiliation{University of Washington}
\author{E.~Blucher}\affiliation{University of Chicago}
\author{D.~Bryman}\affiliation{University of British Columbia}\affiliation{TRIUMF}
\author{S.~Chen}\affiliation { Tsinghua University  }
\author{V.~Cirigliano}\affiliation{Theoretical Division, Los Alamos National Laboratory}%, Los Alamos, NM 87545, USA}
\author{S.~Corrodi}\affiliation{Argonne National Laboratory}
\author{A. Crivellin}\affiliation{Paul Scherrer Institute}\affiliation{University of Zurich}\affiliation{CERN}
\author{S.~Cuen-Rochin}\affiliation{Tec de Monterrey}
\author{A.~DiCanto}\affiliation{Brookhaven National Laboratory}
\author{L.~Doria}\affiliation{Johannes Gutenberg University Mainz}
\author{A.~Gaponenko}\affiliation{Fermilab}
\author{A.~Garcia}\affiliation{University of Washington}
\author{L.~Gibbons}\affiliation{Cornell University}
\author{C.~Glaser}\affiliation {University of Virginia}
\author{M.~Escobar~Godoy}\affiliation {University of California Santa Cruz}
\author{D.~G\"oldi}\affiliation{ETH Zurich}
\author{S.~Gori}\affiliation {University of California Santa Cruz}
\author{T.~Gorringe}\affiliation{University of Kentucky}
\author{D.~Hertzog}\affiliation{University of Washington}
\author{Z.~Hodge}\affiliation{University of Washington}
\author{M.~Hoferichter}\affiliation{University of Bern}
\author{S.~Ito}\affiliation{KEK}
\author{T.~Iwamoto}\affiliation{University of Tokyo}
\author{P.~Kammel}\affiliation{University of Washington}
\author{B.~Kiburg}\affiliation{Fermilab}
\author{K.~Labe}\affiliation{Cornell University}
\author{J.~LaBounty}\affiliation{University of Washington}
\author{U.~Langenegger}\affiliation{Paul Scherrer Institute}
\author{C.~Malbrunot}\affiliation{TRIUMF}
%\author{W. Marciano}\affiliation{Brookhaven National Laboratory}
\author{S.M.~Mazza}\affiliation {University of California Santa Cruz}
\author{S.~Mihara}\affiliation{KEK}
\author{R.~Mischke}\affiliation{TRIUMF}
\author{T.~Mori}\affiliation{University of Tokyo}
\author{J.~Mott}\affiliation{Fermilab}
\author{T.~Numao}\affiliation{TRIUMF}
\author{W.~Ootani}\affiliation{University of Tokyo}
\author{J.~Ott}\affiliation {University of California Santa Cruz}
\author{K.~Pachal}\affiliation{TRIUMF}
\author{C.~Polly}\affiliation{Fermilab}
\author{D.~Po\v{c}ani\'c}\affiliation {University of Virginia}
\author{X.~Qian}\affiliation{Brookhaven National Laboratory}
\author{D.~Ries}\affiliation{Johannes Gutenberg University Mainz}
\author{R.~Roehnelt}\affiliation{University of Washington}
\author{B.~Schumm}\affiliation {University of California Santa Cruz}
\author{P.~Schwendimann}\affiliation{University of Washington}
\author{A.~Seiden}\affiliation {University of California Santa Cruz}
\author{A.~Sher}\affiliation{TRIUMF}
\author{R.~Shrock}\affiliation {Stony Brook University}
\author{A.~Soter}\affiliation{ETH Zurich}
\author{T.~Sullivan}\affiliation{University of Victoria}
\author{M.~Tarka}\affiliation {University of California Santa Cruz}
\author{V.~Tischenko}\affiliation{Brookhaven National Laboratory}
\author{A.~Tricoli}\affiliation{Brookhaven National Laboratory}
\author{B.~Velghe}\affiliation{TRIUMF}

\author{V.~Wong}\affiliation{TRIUMF}
\author{E.~Worcester}\affiliation{Brookhaven National Laboratory}
\author{M.~Worcester}\affiliation{Brookhaven National Laboratory}
\author{C.~Zhang}\affiliation{Brookhaven National Laboratory}
% OPT out
%\author {A. Knecht}%\affiliation{PSI}
%\author {D. Salvat}%\affiliation{Indiana University}
%\author{A.~Czarnecki}\affiliation{University of Alberta}
%\author{D.~Jaffe}\affiliation{Brookhaven National Laboratory}
%\author{S.~Kettel}\affiliation{Brookhaven National Laboratory}
% No response
%\author{T.~Wataru}\affiliation{University of Tokyo}
%\author{A.~Grillo}\affiliation {University of California Santa Cruz}
%\author{M.~Gorchteyn}\affiliation{Johannes Gutenberg University Mainz}
%\author{C.~Ortega Hernandez}\affiliation{Universidad Nacional Autonoma de Mexico}

==> Planning/collaboration.tex <==








\author {W. Altmannshofer, S. Gori, M. Godoy, A. Grillo, S. Mazza, J. Ott,  B. Schumm, A. Seiden, M. Tarka}
\affiliation {University of California Santa Cruz}
\author {H. Binney, A. Garcia, D. Hertzog, Z. Hodge, P. Kammel, J. LaBounty, R. Roehnelt}
\affiliation { University of Washington  }
\author {E. Blucher}
\affiliation{University of Chicago}
\author {D. Bryman}
\affiliation{University of British Columbia  and TRIUMF}
\author {S. Chen}
\affiliation { Tsinghua University  }
\author {V. Cirigliano}
\affiliation{ Los Alamos National Laboratory}%, Los Alamos, NM 87545, USA}
%\author {A. Crivellin}
%\affiliation{Paul Scherrer Institute, University of Zurich}

\author{S. Corrodi}
\affiliation{Argonne National Laboratory}

\author { C. Ortega Hernandez}
\affiliation{Universidad Nacional Autonoma de Mexico}
\author{S. Cuen-Rochin}
\affiliation{Tec de Monterrey}
\author {A. Czarnecki}
\affiliation{University of Alberta}
\author {A. DiCanto, D. Jaffe, S. Kettel,
%W. Marciano, 
V. Tischenko, A. Tricoli, E. Worcester}
\affiliation {Brookhaven National Laborory}
\author {L. Doria, M. Gorchtein, D. Ries}
\affiliation{ Johannes Gutenberg University Mainz}
\author {A. Gaponenko, B. Kiburg,J. Mott, C. Polly}
\affiliation {Fermilab}
\author {L. Gibbons, K. Labe}
\affiliation{Cornell University}
\author {C. Glaser, D. Po\v{c}ani\'c}
\affiliation {University of Virginia}
\author {T. Gorringe}
\affiliation{University of Kentucky}
\author { M. Hoferichter}
\affiliation { University of Bern  }
\author{S.  Ito, S. Mihara}
\affiliation {KEK}
\author {T. Iwamoto, T. Mori, W. Ootani, T. Wataru}
\affiliation {University of Tokyo  }
%\author {A. Knecht, U. Langenegger}
\author {P. Schwendimann, U. Langenegger}
\affiliation{PSI}
\author{ C. Malbrunot}
\affiliation{CERN}
\author { R. Mischke, T. Numao, K. Pachal, A. Sher, B. Velghe, V. Wong}
\affiliation{TRIUMF}
%\author { D. Salvat}
%\affiliation{Indiana University}
\author  {A. Soter}
\affiliation{ETH Zurich}
\author  {R. Shrock}
\affiliation {Stony Brook University}
\author {T. Sullivan}
\affiliation{University of Victoria}


==> SimAnal.tex <==
\subsection {Beam and beam instrumentation}
\subsection {LXe Calorimeter}
\subsection {ATAR}


==> Simulations and Analysis/Introduction.tex <==
Precise low-energy measurements of observables that can be very accurately calculated in the Standard Model (SM)  offer highly sensitive tests of new physics (NP). In light of the existing intriguing hints for lepton flavor universality (LFU) violating NP~\cite{Crivellin:2021sff,Fischer:2021sqw,Bryman:2021teu}, the ratio $R_{e/\mu} = \Gamma(\pi^+\rightarrow e^+\nu(\gamma))/\Gamma(\pi^+\rightarrow \mu^+\nu(\gamma))$ for pion decays to positrons relative to muons is especially promising: %, known theoretically with a precision better than $\unit[0.01]{\%}$,
it is one of the most precisely known observables involving quarks within the SM and NP can even have (chirally) enhanced effects, making it an extremely sensitive probe of NP.
%The branching ratio $R_{e/\mu} = \Gamma(\pi^+\rightarrow \mu+\nu(\gamma))/\Gamma(\pi^+\rightarrow e+\nu(\gamma))$ for pion decays to positrons over muons is a highly sensitive probe for new physics. In the Standard Model (SM), $R_{e/\mu}$ has been calculated with extraordinary precision at the $10^{-4}$ level perhaps the most precisely calculated weak interaction observable involving quarks. 
However, while the uncertainty of the SM calculation for $R_{e/\mu}$ is 
very small (with relative precision $1.2\times 10^{-4}$~\cite{Cirigliano:2007xi}), the current experimental world average is about a factor 15 less precise, limiting the NP reach.
%and the decay $\pi^+\rightarrow e^+\nu$ is helicity suppressed by the $V-A$ structure of charged currents, a measurement of $R_{e/\mu}$ is extremely sensitive to the presence of pseudoscalar (and scalar) couplings absent from the SM; a disagreement with the theoretical expectation would unambiguously imply the existence of NP. Moreover, the comparison of $R_{e/\mu}$ measurements with SM theory already now provides the most accurate measure of lepton universality at the level of $0.1\%$.

A new experiment, PIONEER, is proposed at Paul Scherrer Institute (PSI), where high-intensity pion beams can be delivered. In Phase~I, it  will bridge the gap of a factor 15  between theoretical and experimental precision for $R_{e/\mu}$. With measurements at the $0.01\%$ level in precision, NP up to the PeV scale~\cite{Bryman:2011zz} may be revealed. Such precision would  contribute to  stringent tests of LFU in a context where several intriguing hints of LFU violation (LFUV) have emerged. In addition, it will allow extended searches for exotics such as heavy neutral leptons and dark sector processes. In later Phases (II,III),  PIONEER  will  also study  pion beta decay $\pi^+\to \pi^0 e^+ \nu (\gamma)$ ultimately aiming at  an order of magnitude improvement in precision to determine \vud in a theoretically pristine manner and test CKM unitarity, for which there is presently a $ 3\sigma$ tension~\cite{ParticleDataGroup:2020ssz}. PIONEER is an ambitious program that will span more than a decade of research activity at PSI. With the current proposal we seek approval of the Phase I measurement of $R_{e/\mu}$, so that we can
move forward with applications to  national funding agencies.


While we focus on the measurement of the  \pie~ branching ratio $R_{e/\mu}$, the following sections discuss the theoretical motivation for pursuing the full rare pion decay program.  
Discussions of the \nexp\ detector concepts, simulations, estimated sensitivities, and planning for realization  follow. In the final section, we discuss aspects related to training, equity, diversity and inclusion.
Appendices contain greater detail on some of the topics.

==> Simulations and Analysis/Suppress0.tex <==








With an anticipated tail fraction of f=0.5\% of \pie~ events, $\mu-e$ decays must be suppressed to a level that allows measurement of f with accuracy 1-2\%. This can be accomplished by using ATAR information to identify stopped pions by energy loss, and range-energy relations, using a narrow time window (e.g. 3-35 ns) following the pion stop, observing the 4.2 MeV decay muon, and suppressing events with pion DIF, and muon DIF following pion DAR by tracking and energy loss measurements.

%Suppressing events mimicing $\pi^{+}\rightarrow e^{+}\nu$ decays from  decay-in-flight $\pi^{+} \rightarrow \mu^{+} \nu$ events in the “low energy tail” region. 
As illustrated in Figure \ref{fig:EventTypes}, a background source of $\pi^{+} \rightarrow \mu^{+} \rightarrow  e^{+}$ events comes from pions that decay in flight ($\pi\,\mathrm{DIF}$) either in the ATAR or upstream, followed by muon  decay at rest. 
In addition,  muons that originate from pion DAR in the ATAR can decay in flight before stopping ($\mu\,\mathrm{DIF}$), leaving a positron with the same time distribution as the ones in a $\pi^{+}\rightarrow e^{+}\nu$ events. 
%Table ? indicates the proportions of each types of decay-in-flight events to the decay-at-rest $\pi^{+}\rightarrow e^{+}\nu$ events.
With high granularity and sub-ns timing resolution, the ATAR  can observe the energy deposits of the pion decay products, and thus identifying these different decay modes.
Figure ? shows the distribution of the $\pi$ decay vertex position along the beam direction for the various decay modes of $\pi^{+} \rightarrow \mu^{+} \nu$ events. The individual ATAR event display of some $\pi^{+}\rightarrow e^{+}\nu$ and $\pi^{+} \rightarrow \mu^{+} \rightarrow  e^{+}$ examples are included in Appendix ?. 

Initial studies indicate that the $\pi\,\mathrm{DIF}$ events can be rejected by a suppression factor of 50 using an early decay positron timing window of 5-35 ns (see Figure ?). 
It has been studied with the simulation that the in-ATAR $\pi\,\mathrm{DIF}$ events can be further reduced by a suppression factor of 200 with a traditional cut-based method when the ATAR information is utilized to determine the pion decay position, the existence of kinks in the topology, and dE/dx along the track. 
Under the conservative assumption that 1\% of $\pi^{+}\rightarrow e^{+}\nu$ events would lie in the tail region, this results in an estimation of 0.09 in-ATAR $\pi\,\mathrm{DIF}$ event per $\pi^{+}\rightarrow e^{+}\nu$ event. 
To mitigate the events where the pion decay-in-flight between the degrader and the ATAR, an upstream tracker will be placed right in front of the degrader to provide the tracking of the incoming pion. If the pion decay in flight between the degrader and the ATAR, a non-zero kink angle between the track in the upstream tracker and the one in the ATAR will be detected. This would highly suppress the upstream $\pi\,\mathrm{DIF}$ events.

For the $\mu\,\mathrm{DIF}$ event, although the probability of occurrence is much smaller, it had been a dominating source of tail corrections in previous experiment, as it has the same decay positron time distribution. Thanks to the high granularity of the ATAR, it is possible to set apart the energy deposition of the closely-happening muon and positron, or even measure their energy loss along the decay length. It is expected that a muon decays in roughly 1 mm, and thus leaving hits in 4 strips on average. From a simulation of $\mu\,\mathrm{DIF}$ events, a suppression factor of 18 was recognized with the separation power from dE/dx measurement. This leads to 0.08 $\mu\,\mathrm{DIF}$ events per $\pi^{+}\rightarrow e^{+}\nu$ event. As a whole, the simulation studies indicate that all the $\mathrm{DIF}$ background events together could be suppressed to a level of 10\% or smaller, allowing the experiment to achieve a tail correction uncertainty as low as 1\%.

\begin{itemize}
  \item For upstream $\pi\,\mathrm{DIF}$ event, hopefully we will have some numbers to update. Otherwise, maybe we can try to quote a conservative number from PIENU’s experience. 
  \item For $\mu\,\mathrm{DIF}$ event, we might update some numbers after seeing how kink topology might help as well.
\end{itemize}



==> TrainingEDI.tex <==
During the development and operation of \nexp~   particular attention will be given to maintain diversity including women and other under-represented groups as well as  in  the level of experience of the participants.  Mentorship is also an important part of the training of highly qualified personnel (HQP). Both mentors and mentees benefit from a larger group of HPQs and PIs with/from whom they can  interact, learn, and teach. Thus, it is important to have a well-balanced team of HQP and principals (PI). 


The diversity of experience is also reflected in the current PI team including very experienced PIs and early to mid-career researchers.
All PIs have significant experience in training HQP and several members have followed  training courses related to Equity, Diversity and Inclusion (EDI) aspects of supervision and have been  active in outreach in view of improving gender-balance in science. The recruitment and inclusion of women and under‐representative minorities in the PIONEER  group is a priority and the participant groups have good records. 
%\footnote{For example, 45\% of the graduate students and postdoctoral researchers hired by the rare decay group at TRIUMF/UBC since 2000 were either women or under‐represented minorities and  two female TRIUMF faculty members recently joined the group.}

We commit to providing equitable mentorship with the intention of advancing the research objectives of the group and the personal objectives of the participants. Opportunities to participate in diversity, inclusion, and equity activities as well as soft-skill and cross-sectoral training will be encouraged.

Students and PDFs will be given opportunities to present their work at conferences and collaboration meetings. Since the pandemic started many conferences turned to an online or hybrid format. While in-person meetings remain important for networking and informal idea exchanges, maintaining the pre-covid level of travel for conferences should be carefully assessed in light of environmental impact and equal opportunities for HQP. A report from  ECFA (European Committee for Future Accelerators) early career scientist panel meant as input to the 2020 European Strategy Update for particle physics (https://arxiv.org/abs/2002.02837) raised concerns about the carbon-footprint of conference-related travels and the discriminatory effect that in-person only meetings have on scientists with children (having unfortunately still a more important impact on female scientists). Thus, as far as possible, we will leave the option to the HQP to decide on an in-person or remote attendance to meetings and conferences.

The HQP in the groups will be part of an international collaboration of currently 25 research institutes and universities across USA, Europe, Canada, Japan, China and Mexico, offering many opportunities for networking in a diverse environment.
 
As far as research training is concerned, PIONEER, being a medium scale precision physics experiment, offers excellent opportunities for advanced hands-on training on a wide variety of hardware and software technologies (LXe calorimetry, cryogenic engineering, photo detectors, advanced Si detectors, state-of-the-art data acquisition, high speed electronics). Those will be complemented with training in sophisticated data analysis and simulation methods applicable to many forefront areas of experimental science but also to  industry where those skills are highly sought. 

Students and early researchers will be provided the opportunity to learn about all aspects of  the experiment leading to well rounded training for future careers in particle physics and other technical pursuits.
Students and postdoctoral researchers will take on significant and diverse individual responsibilities making them able to move to other leading high energy physics projects like the LHC, to low energy nuclear physics projects, or to industry. The experienced members of the team will mentor and instruct the more junior members in a collegial atmosphere which encourages learning and accomplishment.
Within this project, the PDF and  students will experience both the large infrastructure laboratories  and the university lab environments . They will also  work on R\&D developments and on simulations providing them with hardware and computational projects. Students will participate in the design of test assemblies, installation and data-taking  as well as data-analysis.
Some will be focusing on  simulation studies and machine-learning analyses.  


In summary HQPs on this project will benefit from an inclusive environment and the supervision of a strong group of PIs with a wide range of expertise incorporated within a larger group of experts. 

